On Margulis cusps of hyperbolic 4-manifolds

We study the geometry of the Margulis region associated with an irrational screw translation $g$ acting on the 4-dimensional real hyperbolic space. This is an invariant domain with the parabolic fixed point of $g$ on its boundary which plays the role of an invariant horoball for a translation in dimensions $\leq 3$. The boundary of the Margulis region is described in terms of a function $B_\alpha : [0,\infty) \to {\mathbb R}$ which solely depends on the rotation angle $\alpha \in {\mathbb R}/{\mathbb Z}$ of $g$. We obtain an asymptotically universal upper bound for $B_\alpha(r)$ as $r \to \infty$ for arbitrary irrational $\alpha$, as well as lower bounds when $\alpha$ is Diophatine and the optimal bound when $\alpha$ is of bounded type. We investigate the implications of these results for the geometry of Margulis cusps of hyperbolic 4-manifolds that correspond to irrational screw translations acting on the universal cover. Among other things, we prove bi-Lipschitz rigidity of these cusps.

==> psbox.tex <==
%% Every macro likes a little privacy...
\catcode`\@=11


                  %% -------------------------- %%


%%
%% Trying to tame the variety of \special commands for Postscript: the
%% universal internal command \PSspeci@l##1##2 takes ##1 to be the
%% filename and ##2 to be the integer scale factor*1000 (as for usual
%% TeX \scale commands)
%

\def\psfortextures{%     For TeXtures on the Macintosh
\def\PSspeci@l##1##2{%
\special{illustration ##1\space scaled ##2}}}

                          %% ----------- %%

\def\psfordvips{%      For DVIPS converter on VAX, UNIX and PC's
\def\PSspeci@l##1##2{%
\d@my=0.1bp \d@mx=\drawingwd \divide\d@mx by\d@my%
\special{PSfile=##1\space llx=\psllx\space lly=\pslly\space%
urx=\psurx\space ury=\psury\space rwi=\number\d@mx}}}

                          %% ----------- %%

%%
%% Correspond parfaitement a la doc OzTeX.
%% 
\def\psforoztex{%        For the OzTeX shareware on the Macintosh
\def\PSspeci@l##1##2{%
\special{##1 \space
      ##2 1000 div dup scale
      \putsp@ce{\number-\psllx} \putsp@ce{\number-\pslly} translate}}}
\def\putsp@ce#1{#1 }

                          %% ----------- %%

\def\psonlyboxes{%     Draft-like behaviour if none of the others works
\def\PSspeci@l##1##2{%
\at{0cm}{0cm}{\boxit{\vbox to\drawinght
  {\vss
  \hbox to\drawingwd{\at{0cm}{0cm}{\hbox{(##1)}}\hss}
  }}}}}


                  %% -------------------------- %%


%%
%% \ReadPSize{PSfilename} reads the dimensions of a PostScript drawing
%% and stores it in \drawinght(wd)
%%
\newdimen\drawinght\newdimen\drawingwd
\newdimen\psxoffset\newdimen\psyoffset
\newbox\drawingBox

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%%
\pspoints=1bp          % Adobe points are `big'
\epsfxsize=0pt         % Default value, means `use natural size'
\epsfysize=0pt         % ditto


\def\ReadPSize#1{
\edef\PSfilename{#1}
\global\def\epsfllx{72}
\global\def\epsflly{72}
\global\def\epsfurx{540}
\global\def\epsfury{720}
%%
%%   The first thing we need to do is to open the
%%   PostScript file, if possible.
%%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%%
%%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%%   start with %. We're looking for the bounding box comment.
%%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%%
%%   We check to see if the first character is a % sign;
%%   if not, we stop reading (unless the line was entirely blank);
%%   if so, we look further and stop only if the line begins with
%%   `%%BoundingBox:'.
%%
          \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi
\def\psllx{\epsfllx}\def\pslly{\epsflly}%
\def\psurx{\epsfurx}\def\psury{\epsfury}%
%% Units related by crazy factors as bp/pt=72.27/72 should be BANNED!
\drawinght=\epsfury bp%
\advance\drawinght by-\epsflly bp%
\drawingwd=\epsfurx bp%
\advance\drawingwd by-\epsfllx bp%
}

%%
%%   We still need to define the tricky \epsfaux macro. This requires
%%   a couple of magic constants for comparison purposes.
%%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%%
%%   So we're ready to check for `%BoundingBox:' and to grab the
%%   values if they are found.
%%
%% \long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
%%    \def\testit{#2}\ifx\testit\epsfbblit
%%       \epsfgrab #3 . . . \\%
%%       \epsffileokfalse
%%       \global\epsfbbfoundtrue
%%    \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 @ @ @ \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
   \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%

%%
%%   Here we grab the values and stuff them in the appropriate definitions.
%%
%% \def\epsfgrab #1 #2 #3 #4 #5\\{%
%%    \global\def\epsfllx{#1}\ifx\epsfllx\empty
%%       \epsfgrab #2 #3 #4 #5 .\\\else
%%    \global\def\epsflly{#2}%
%%    \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
   \global\def\epsfllx{#1}\ifx\epsfllx\empty
      \epsfgrab #2 #3 #4 #5 @\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%


                  %% -------------------------- %%


%%
%% \psboxto(xdim;ydim){psfilename}: you specify the dimensions and
%%    TeX uniformly scales to fit the largest one. If xdim=0pt, the
%%    scale is fully determined by ydim and vice versa.
%%    Notice: psboxes are a real vboxes; couldn't take hbox otherwise all
%%    indentation and all cr's would be interpreted as spaces (hugh!).
%%
\newcount\xscale \newcount\yscale \newdimen\pscm\pscm=1cm
\newdimen\d@mx \newdimen\d@my
\let\ps@nnotation=\relax
\def\psboxto(#1;#2)#3{\vbox{
   \catcode`\:=12
   \ReadPSize{#3}
   \divide\drawingwd by 1000
   \divide\drawinght by 1000
   \d@mx=#1
   \ifdim\d@mx=0pt\xscale=1000
         \else \xscale=\d@mx \divide \xscale by \drawingwd\fi
   \d@my=#2
   \ifdim\d@my=0pt\yscale=1000
         \else \yscale=\d@my \divide \yscale by \drawinght\fi
   \ifnum\yscale=1000
         \else\ifnum\xscale=1000\xscale=\yscale
                    \else\ifnum\yscale<\xscale\xscale=\yscale\fi
              \fi
   \fi
   \divide \psxoffset by 1000\multiply\psxoffset by \xscale
   \divide \psyoffset by 1000\multiply\psyoffset by \xscale
   \global\divide\pscm by 1000
   \global\multiply\pscm by\xscale
   \multiply\drawingwd by\xscale \multiply\drawinght by\xscale
   \ifdim\d@mx=0pt\d@mx=\drawingwd\fi
   \ifdim\d@my=0pt\d@my=\drawinght\fi
\message{[#3\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
 \hbox to\d@mx{\hss\vbox to\d@my{\vss
   \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
      \kern-\psyoffset
      \PSspeci@l{\PSfilename}{\the\xscale}
      \vss}\hss\ps@nnotation}
   \global\ht\drawingBox=\the\drawinght
   \global\wd\drawingBox=\the\drawingwd
   \baselineskip=0pt
   \copy\drawingBox
 \vss}\hss}
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%% \psboxscaled{scalefactor*1000}{PSfilename} allows to bypass the
%%   rounding errors of TeX integer divisions for situations where the
%%   TeX box should fit the original BoundingBox with a precision better
%%   than 1/1000.
%%
\def\psboxscaled#1#2{\vbox{
  \catcode`\:=12
  \ReadPSize{#2}
  \xscale=#1
  \divide\drawingwd by 1000\multiply\drawingwd by\xscale
  \divide\drawinght by 1000\multiply\drawinght by\xscale
  \divide \psxoffset by 1000\multiply\psxoffset by \xscale
  \divide \psyoffset by 1000\multiply\psyoffset by \xscale
  \global\divide\pscm by 1000
  \global\multiply\pscm by\xscale
\message{[#2\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
  \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
     \kern-\psyoffset
     \PSspeci@l{\PSfilename}{\the\xscale}
     \vss}\hss\ps@nnotation}
  \global\ht\drawingBox=\the\drawinght
  \global\wd\drawingBox=\the\drawingwd
  \baselineskip=0pt
  \copy\drawingBox
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%%  \psbox{PSfilename} makes a TeX box having the minimal size to
%%      enclose the picture
\def\psbox#1{\psboxscaled{1000}{#1}}


                  %% -------------------------- %%

%%
%%  Annotations & Captions etc...
%%
%% \centinsert{anybox} is just a centered \midinsert, but is included as
%% people barely use the original inserts from TeX.
%%
\def\centinsert#1{\midinsert\line{\hss#1\hss}\endinsert}
\def\psannotate#1#2{\def\ps@nnotation{#2\global\let\ps@nnotation=\relax}#1}
\def\pscaption#1#2{\vbox{
   \setbox\drawingBox=#1
   \copy\drawingBox
   \vskip\baselineskip
   \vbox{\hsize=\wd\drawingBox\setbox0=\hbox{#2}
     \ifdim\wd0>\hsize
       \noindent\unhbox0\tolerance=5000
    \else\centerline{\box0}
    \fi
}}}


                  %% -------------------------- %%


%%
%% \at{#1}{#2}{#3} puts #3 at #1-higher and #2-right of the current
%%    position without moving it (to be used in annotations).
%%
\def\at#1#2#3{\setbox0=\hbox{#3}\ht0=0pt\dp0=0pt
  \rlap{\kern#1\vbox to0pt{\kern-#2\box0\vss}}}


                  %% -------------------------- %%


%%
%% \gridfill(ht;wd) makes a 1cm*1cm grid of ht by wd whose lower-left
%%   corner is the current point
%%
\newdimen\gridht \newdimen\gridwd
\def\gridfill(#1;#2){
  \setbox0=\hbox to 1\pscm
  {\vrule height1\pscm width.4pt\leaders\hrule\hfill}
  \gridht=#1
  \divide\gridht by \ht0
  \multiply\gridht by \ht0
  \advance \gridht by \ht0
  \gridwd=#2
  \divide\gridwd by \wd0
  \multiply\gridwd by \wd0
  \advance \gridwd by \wd0
  \vbox to \gridht{\leaders\hbox to\gridwd{\leaders\box0\hfill}\vfill}}


                  %% -------------------------- %%


%%
%% Useful to measure where to put annotations
%%
\def\fillinggrid{\at{0cm}{0cm}{\vbox{\gridfill(\drawinght;\drawingwd)}}}


                  %% -------------------------- %%


%%
%% \frameit{\thick}{\skip}{\anybox}
%%    draws with thickness \thick a box around \anybox, leaving \skip of
%%    blank around it. eg \frameit{0.5pt}{1pt}{\hbox{hello}}
%% \boxit{\anybox} is a shortcut.
%%
\def\frameit#1#2#3{\hbox{\vrule width#1\vbox{
  \hrule height#1\vskip#2\hbox{\hskip#2\vbox{#3}\hskip#2}%
        \vskip#2\hrule height#1}\vrule width#1}}
\def\boxit#1{\frameit{0.4pt}{0pt}{#1}}


                  %% -------------------------- %%


\catcode`\@=12 % cs containing @ are unreachable
%\catcode`\@=\active % cs containing @ are unreachable
 


